A Deep, Information-theoretic Framework for Robust Biometric Recognition

Deep neural networks (DNN) have been a de facto standard for nowadays biometric recognition solutions. A serious, but still overlooked problem in these DNN-based recognition systems is their vulnerability against adversarial attacks. Adversarial attacks can easily cause the output of a DNN system to greatly distort with only tiny changes in its input. Such distortions can potentially lead to an unexpected match between a valid biometric and a synthetic one constructed by a strategic attacker, raising security issue. In this work, we show how this issue can be resolved by learning robust biometric features through a deep, information-theoretic framework, which builds upon the recent deep variational information bottleneck method but is carefully adapted to biometric recognition tasks. Empirical evaluation demonstrates that our method not only offers stronger robustness against adversarial attacks but also provides better recognition performance over state-of-the-art approaches.

==> tables/beta.tex <==
\begin{table}[h!]
  \centering
  \caption{The effect of different $\beta$ in the MNIST dataset.}
    \begin{tabular}{lcccc}
    \toprule
        $\beta$  & $1 \times 10^{-4}$ & $1 \times 10^{-3}$ &  $1 \times 10^{-2}$  & $1 \times 10^{-1}$  \\
    \midrule
    RI  &  2.2214& 2.0119& 1.9867& 2.2437\\
    \midrule
    EER  &  0.9994&  0.9991& 0.9989 & 0.9989\\
    \bottomrule
    \end{tabular}%
  \label{table:beta}%
\end{table}%



% \begin{table*}
%   \centering
%   \caption{The sensitivity w.r.t $\beta$.}
%     \begin{tabular}{lccccc}
%     \toprule
%         $\beta$  & $1 \times 10^{-5}$  & $1 \times 10^{-4}$ & $1 \times 10^{-3}$ &$1 \times 10^{-2}$ &$1 \times 10^{-1}$ \\
%     \midrule
%     MADR  &2.1087&  2.2214& 2.0119& 1.9867& 2.2437\\
%     \midrule
%     AUC  &0.9989&  0.9994&  0.9991& 0.9989 & 0.9989\\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:t1}%
% \end{table*}%

==> tables/dataset.tex <==
\begin{table}[h!]
  \centering
  \caption{A summary of CASIA-webface and LFW dataset.}
    \begin{tabular}{lcc}
    \toprule
         & num. of individuals & num. of images  \\
    \midrule
    CASIA-Webface  & 10575 & 494414  \\
    \midrule
    LFW  & 5749 & 13233  \\
    \bottomrule
    \end{tabular}%
  \label{table:dataset}%
\end{table}%

==> tables/table-LFWV.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{lc}
    \toprule
          & 10Flod-ACC \\
    \midrule
    Softmax & \multicolumn{1}{l}{0.9620+0.0106} \\
    DVIB  & \multicolumn{1}{l}{0.9797+0.0073} \\
    Center & \multicolumn{1}{l}{0.9798+0.0082} \\
    L2 const. & \multicolumn{1}{l}{0.9798+0.0331} \\
    SphereF. & \multicolumn{1}{l}{0.9810+0.0099} \\
    VSP-advt & \textbf{0.9852+0.0059} \\
    \bottomrule
    \end{tabular}%
  \label{tab:t4}%
\end{table}%


==> tables/table-cnn20.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet4'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{crc}
%     \toprule
%     \multirow{4}[4]{*}{Stage1} & Conv(64,3,2,1) & \multirow{2}[2]{*}{x1} \\
%           & pReLU &  \\
% \cmidrule{2-3}          & Conv(64,3,1,1) & \multirow{2}[2]{*}{x2,SC/2} \\
%           & pReLU &  \\
%     \midrule
%     \multirow{4}[4]{*}{Stage2} & Conv(128,3,2,1) & \multirow{2}[2]{*}{x1} \\
%           & pReLU &  \\
% \cmidrule{2-3}          & Conv(128,3,1,1) & \multirow{2}[2]{*}{x2, SC/2} \\
%           & pReLU &  \\
%     \midrule
%     \multirow{4}[4]{*}{Stage3} & Conv(256,3,2,1) & \multirow{2}[2]{*}{x1} \\
%           & pReLU &  \\
% \cmidrule{2-3}          & Conv(256,3,1,1) & \multirow{2}[2]{*}{x8, SC/2} \\
%           & pReLU &  \\
%     \midrule
%     \multirow{4}[4]{*}{Stage4} & Conv(512,3,2,1) & \multirow{2}[2]{*}{x1} \\
%           & pReLU &  \\
% \cmidrule{2-3}          & Conv(512,3,1,1) & \multirow{2}[2]{*}{x2, SC/2} \\
%           & pReLU &  \\
%     \midrule
%     Output & FC(1024) & x1 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:t2}%
% \end{table}%
% Table generated by Excel2LaTeX from sheet 'Sheet4'
% Table generated by Excel2LaTeX from sheet 'Sheet4'


% \begin{table*}[t]
%  % Table generated by Excel2LaTeX from sheet 'Sheet4'
%   \centering
%   \caption{Detailed network architecture of the CNN employed in the experiments. }
%     \begin{tabular}{lp{2.945em}lp{2.72em}lp{2.61em}lp{2.61em}l}
%     \hline
%     \multicolumn{2}{c}{Stage1} & \multicolumn{2}{c}{Stage2} & \multicolumn{2}{c}{Stage3} & \multicolumn{2}{c}{Stage4} & \multicolumn{1}{c}{Output} \\
%     \hline
%     Conv(64,3,2,1) & \multicolumn{1}{l}{\multirow{2}[2]{*}{x1}} & Conv(128,3,2,1) & \multicolumn{1}{l}{\multirow{2}[2]{*}{x1}} & Conv(256,3,2,1) & \multicolumn{1}{l}{\multirow{2}[2]{*}{x1}} & Conv(512,3,2,1) & \multicolumn{1}{l}{\multirow{2}[2]{*}{x1}} & \multirow{4}[4]{*}{FC(1024)}\\
%     pReLU & \multicolumn{1}{l}{} & pReLU & \multicolumn{1}{l}{} & pReLU & \multicolumn{1}{l}{} & pReLU & \multicolumn{1}{l}{} &  \\
% \cline{1-8}    Conv(64,3,1,1) & x2    & Conv(128,3,1,1) & x2    & Conv(256,3,1,1) & x8    & Conv(512,3,1,1) & x2    &  \\
%     pReLU & SC/2  & pReLU & SC/2  & pReLU & SC/2  & pReLU & SC/2  & \\
%     \hline
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table*}



\begin{table*}[h]
 % Table generated by Excel2LaTeX from sheet 'Sheet4'
  \centering
  \caption{Detailed network architecture of the CNN employed in the experiments. }
    \begin{tabular}{lllll}
    \hline
    \quad Stage 1  & \quad Stage 2 \quad & \quad Stage 3 \quad & \quad Stage 4 \quad &  Stage 5 \quad \\
    \hline
    Conv(64,3,2,1) \quad & \quad Conv(128,3,2,1) \quad & \quad Conv(256,3,2,1) \quad & \quad Conv(512,3,2,1) \quad &  \multirow{6}{*}{FC(1024)}  \\
    pReLU & \quad pReLU  \quad &  \quad pReLU \quad & \quad pReLU \quad  &  \\
    x1, No SC \quad & \quad x1, No SC  \quad &  \quad x1, No SC \quad & \quad x1, No SC \quad & \\
\cline{1-4}    
Conv(64,3,1,1)     &  \quad  Conv(128,3,1,1) \quad  &    \quad   Conv(256,3,1,1)  \quad    & \quad  Conv(512,3,1,1)  \quad    &  \\
     pReLU & \quad pReLU  \quad &  \quad pReLU \quad & \quad pReLU \quad  &  \\
     x2, SC/2 \quad & \quad x2, SC/2  \quad &  \quad x2, SC/2 \quad & \quad x2, SC/2 \quad & \\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}



